How to assign volunteers to tasks compatibly ? A graph theoretic and parameterized approach

In this paper we study a resource allocation problem that encodes correlation between items in terms of \conflict and maximizes the minimum utility of the agents under a conflict free allocation. Admittedly, the problem is computationally hard even under stringent restrictions because it encodes a variant of the {\sc Maximum Weight Independent Set} problem which is one of the canonical hard problems in both classical and parameterized complexity. Recently, this subject was explored by Chiarelli et al.~[Algorithmica'22] from the classical complexity perspective to draw the boundary between {\sf NP}-hardness and tractability for a constant number of agents. The problem was shown to be hard even for small constant number of agents and various other restrictions on the underlying graph. Notwithstanding this computational barrier, we notice that there are several parameters that are worth studying: number of agents, number of items, combinatorial structure that defines the conflict among the items, all of which could well be small under specific circumstancs. Our search rules out several parameters (even when taken together) and takes us towards a characterization of families of input instances that are amenable to polynomial time algorithms when the parameters are constant. In addition to this we give a superior $2^{m}|I|^{\Co{O}(1)}$ algorithm for our problem where $m$ denotes the number of items that significantly beats the exhaustive $\Oh(m^{m})$ algorithm by cleverly using ideas from FFT based fast polynomial multiplication; and we identify simple graph classes relevant to our problem's motivation that admit efficient algorithms.

==> Table.tex <==
% !TEX root = main.tex

\definecolor{olivegreen}{rgb}{.8,1,.8}
\newcommand{\tick}{{\color{olivegreen}{\bf \checkmark}}}
\newcommand{\cross}{{\color{red}{\ensuremath{\times}}}}
%\newcommand{\dash}{\leftrightline}


%\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightCyan}{rgb}{0.88,.8,.9}

\definecolor{lightred}{rgb}{1,.8,.8}

\newcolumntype{a}{>{\columncolor{LightCyan}}c}
\newcolumntype{b}{>{\columncolor{LightCyan}}c}
\newcolumntype{d}{>{\columncolor{LightCyan}}c}
\newcolumntype{e}{>{\columncolor{LightCyan}}c}


%\newcommand{\Cy}[1]{{\textcolor{LightCyan}{#1}}}
\newcommand{\Cy}[1]{{\textcolor{LightCyan}{#1}}}

\newcommand{\dash}{\cellcolor{yellow}}


\begin{table*}[htp]
\begin{center}
\begin{tabular}{|c|c|b |c|d|d|c|}
\hline
Utility Functions & \multicolumn{3}{c|}{Arbitrary}& \multicolumn{2}{c|}{Uniform} & Arbitrary \\
\hline
\diagbox{Parameters}{\Co{G}} & Arbitrary & Complete & Cluster & Cluster(2 cliques)&Regular(degree is $m-2$)& \mwisg is \fpt wrt $k$ \\
\hline
{\sf \#agents} & \cellcolor{lightred} \cite{deuermeyer1982scheduling} & & \cellcolor{lightred}{\bf Obs.}~\ref{obs:cluster-2agent}& & & \cellcolor{lightred}\cite{deuermeyer1982scheduling}\\
{\sf \#items} & \cellcolor{olivegreen} {\bf Thm.}\,\ref{thm:fpt-with-items} & & \dash & & &\dash \\
{\sf bundleSize} & \cellcolor{lightred}~{\bf Thm.}\,\ref{thm:nph-edgeless} & & \cellcolor{lightred}~ {\bf Thm.}\,\ref{thm:hardnessForcluster} & & &\cellcolor{lightred}{\bf Thm.} \ref{thm:nph-edgeless}\\
$\eta$ & \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & {\bf ?} & & &{\bf ?}\\
${\sf \#agents} + {\sf bundleSize}$& \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & \cellcolor{olivegreen}~\bf{Thm.}\ref{thm:equiavlence} & & & \cellcolor{olivegreen}~{\bf Thm.}\,\ref{thm:equiavlence} \\
${\sf \# agents} + {\sf bundleSize}+ \eta$ & \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & \dash & & & \dash \\
 $t$ & \cellcolor{olivegreen}~{\bf Thm.}\,\ref{thm:fpt-t} &  & \dash & & & \dash \\
\hline
\end{tabular}
\end{center}
\caption{Summary of our results of \cffa, where the conflict graph belong to the family $\Co{G}$. \Cy{Lavender}  cell represents polynomial time complexity; {\color{olivegreen} Green} cell and {\color{lightred} Pink} cell denote that the 
problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively; white cells with {\bf ?} mark denote that the complexity is open; and {\color{yellow} Yellow} cell denote that the respective parameters are not interesting as the problem is either \fpt w.r.t. smaller parameter or for more general graph class.}
\label{tab:results}
\end{table*}%


%\begin{table*}[htp]
%\begin{center}
%\begin{tabular}{|c|c|b |c|c|}
%\hline
%Parameters & Arbitrary & Complete & Cluster & G is {\sf fpt} wrt k \\
%\hline
%\#agents & \cross \cite{deuermeyer1982scheduling} & & \cross {\bf Obs.}~\ref{obs:cluster-2agent}& \cross \cite{deuermeyer1982scheduling}\\
%\#items & \tick~ {\bf Thm.}\,\ref{thm:fpt-with-items} & & \dash & \dash \\
%bundle size & \cross~{\bf Thm.}\,\ref{thm:nph-edgeless} & & \cross~ {\bf Th.}\,\ref{thm:hardnessForcluster} & \cross \\
%$\eta$ & \cross {\bf Obs.}~\ref{obs:wh-eta} & & ? & ?\\
%$\text{\# agents} + \text{bundlesize}$& \cross & & \tick~\bf{Thm.}\ref{thm:equiavlence} & \tick~{\bf Thm.}\,\ref{thm:equiavlence} \\
%$\text{\# agents} + \text{bundlesize} + \eta$ & \cross & & \dash & \dash \\
%distance from $K_{n}$ & \tick~{\bf Thm.}\,\ref{thm:fpt-t} & \dash & \dash & \dash \\
%\hline
%\end{tabular}
%\end{center}
%\caption{\Cy{Light Cyan} represents polynomial time complexity; \tick\ and \cross\ mean the 
%problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively.}
%
%\label{default}
%\end{table*}%


==> Table_2.tex <==
% !TEX root = main.tex

\definecolor{olivegreen}{rgb}{.8,1,.8}
\newcommand{\tick}{{\color{olivegreen}{\bf \checkmark}}}
\newcommand{\cross}{{\color{red}{\ensuremath{\times}}}}
%\newcommand{\dash}{\leftrightline}


%\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightCyan}{rgb}{0.88,.8,.9}

\definecolor{lightred}{rgb}{1,.8,.8}

\newcolumntype{a}{>{\columncolor{LightCyan}}c}
\newcolumntype{b}{>{\columncolor{LightCyan}}c}
\newcolumntype{d}{>{\columncolor{LightCyan}}c}
\newcolumntype{e}{>{\columncolor{LightCyan}}c}


%\newcommand{\Cy}[1]{{\textcolor{LightCyan}{#1}}}
\newcommand{\Cy}[1]{{\textcolor{LightCyan}{#1}}}

\newcommand{\dash}{\cellcolor{yellow}}


%\begin{table*}[htp]
%\begin{center}
%\begin{tabular}{|c|c|b |c|d|d|c|}
%\hline
%Utility Functions & \multicolumn{3}{c|}{Arbitrary}& \multicolumn{2}{c|}{Uniform} & Arbitrary \\
%\hline
%\diagbox{Parameters}{\Co{G}} & Arbitrary & Complete & Cluster & Cluster(2 cliques)&Regular(degree $n-2$)& \mwisg is \fpt wrt $k$ \\
%\hline
%{\sf \#agents} & \cellcolor{lightred} \cite{deuermeyer1982scheduling} & & \cellcolor{lightred}{\bf Obs.}~\ref{obs:cluster-2agent}& & & \cellcolor{lightred}\cite{deuermeyer1982scheduling}\\
%{\sf \#items} & \cellcolor{olivegreen} {\bf Thm.}\,\ref{thm:fpt-with-items} & & \dash & & &\dash \\
%{\sf bundleSize} & \cellcolor{lightred}~{\bf Thm.}\,\ref{thm:nph-edgeless} & & \cellcolor{lightred}~ {\bf Thm.}\,\ref{thm:hardnessForcluster} & & &\cellcolor{lightred}{\bf Thm.} \ref{thm:nph-edgeless}\\
%$\eta$ & \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & {\bf ?} & & &{\bf ?}\\
%${\sf \#agents} + {\sf bundleSize}$& \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & \cellcolor{olivegreen}~\bf{Thm.}\ref{thm:equiavlence} & & & \cellcolor{olivegreen}~{\bf Thm.}\,\ref{thm:equiavlence} \\
%${\sf \# agents} + {\sf bundleSize}+ \eta$ & \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & \dash & & & \dash \\
% $t$ & \cellcolor{olivegreen}~{\bf Thm.}\,\ref{thm:fpt-t} &  & \dash & & & \dash \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Summary of our results of \cffa, where the conflict graph belong to the family $\Co{G}$. \Cy{Lavender}  cell represents polynomial time complexity; {\color{olivegreen} Green} cell and {\color{lightred} Pink} cell denote that the 
%problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively; white cells with {\bf ?} mark denote that the complexity is open; and {\color{yellow} Yellow} cell denote that the respective parameters are not interesting as the problem is either \fpt w.r.t. smaller parameter or for more general graph class.}
%\definecolor{darkyw}{rgb}{0.8,0.6,0}
\begin{figure*}[t!]
%\begin{subfigure}{6cm}
\centering\includegraphics[width=17cm,height=3.8cm]{table_fig}
\caption{Summary of our results of \cffa, where the conflict graph belongs to the family $\Co{G}$. {\bf \Cy{Lavender}}  cell represents polynomial time complexity; {\color{olivegreen} {\bf Green}} cell and {\color{lightred} {\bf Pink}} cell denote that the 
problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively; white cells with {\bf ?} mark denotes that the complexity is open; and the {\color{yellow} {\bf Yellow}} cell denotes that the respective parameters are not interesting as the problem is either \fpt w.r.t. smaller parameter or for a more general graph class.}
\label{tab:results}
\end{figure*}%


%\begin{table*}[htp]
%\begin{center}
%\begin{tabular}{|c|c|b |c|c|}
%\hline
%Parameters & Arbitrary & Complete & Cluster & G is {\sf fpt} wrt k \\
%\hline
%\#agents & \cross \cite{deuermeyer1982scheduling} & & \cross {\bf Obs.}~\ref{obs:cluster-2agent}& \cross \cite{deuermeyer1982scheduling}\\
%\#items & \tick~ {\bf Thm.}\,\ref{thm:fpt-with-items} & & \dash & \dash \\
%bundle size & \cross~{\bf Thm.}\,\ref{thm:nph-edgeless} & & \cross~ {\bf Th.}\,\ref{thm:hardnessForcluster} & \cross \\
%$\eta$ & \cross {\bf Obs.}~\ref{obs:wh-eta} & & ? & ?\\
%$\text{\# agents} + \text{bundlesize}$& \cross & & \tick~\bf{Thm.}\ref{thm:equiavlence} & \tick~{\bf Thm.}\,\ref{thm:equiavlence} \\
%$\text{\# agents} + \text{bundlesize} + \eta$ & \cross & & \dash & \dash \\
%distance from $K_{n}$ & \tick~{\bf Thm.}\,\ref{thm:fpt-t} & \dash & \dash & \dash \\
%\hline
%\end{tabular}
%\end{center}
%\caption{\Cy{Light Cyan} represents polynomial time complexity; \tick\ and \cross\ mean the 
%problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively.}
%
%\label{default}
%\end{table*}%


==> Table__pallavi_jain_s_conflicted_copy_2023-04-25_.tex <==
% !TEX root = main.tex

\definecolor{olivegreen}{rgb}{.8,1,.8}
\newcommand{\tick}{{\color{olivegreen}{\bf \checkmark}}}
\newcommand{\cross}{{\color{red}{\ensuremath{\times}}}}
%\newcommand{\dash}{\leftrightline}


%\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightCyan}{rgb}{0.88,.8,.9}

\definecolor{lightred}{rgb}{1,.8,.8}

\newcolumntype{a}{>{\columncolor{LightCyan}}c}
\newcolumntype{b}{>{\columncolor{LightCyan}}c}
\newcolumntype{d}{>{\columncolor{LightCyan}}c}
\newcolumntype{e}{>{\columncolor{LightCyan}}c}


%\newcommand{\Cy}[1]{{\textcolor{LightCyan}{#1}}}
\newcommand{\Cy}[1]{{\textcolor{LightCyan}{#1}}}

\newcommand{\dash}{\cellcolor{yellow}}


%\begin{table*}[htp]
%\begin{center}
%\begin{tabular}{|c|c|b |c|d|d|c|}
%\hline
%Utility Functions & \multicolumn{3}{c|}{Arbitrary}& \multicolumn{2}{c|}{Uniform} & Arbitrary \\
%\hline
%\diagbox{Parameters}{\Co{G}} & Arbitrary & Complete & Cluster & Cluster(2 cliques)&Regular(degree $n-2$)& \mwisg is \fpt wrt $k$ \\
%\hline
%{\sf \#agents} & \cellcolor{lightred} \cite{deuermeyer1982scheduling} & & \cellcolor{lightred}{\bf Obs.}~\ref{obs:cluster-2agent}& & & \cellcolor{lightred}\cite{deuermeyer1982scheduling}\\
%{\sf \#items} & \cellcolor{olivegreen} {\bf Thm.}\,\ref{thm:fpt-with-items} & & \dash & & &\dash \\
%{\sf bundleSize} & \cellcolor{lightred}~{\bf Thm.}\,\ref{thm:nph-edgeless} & & \cellcolor{lightred}~ {\bf Thm.}\,\ref{thm:hardnessForcluster} & & &\cellcolor{lightred}{\bf Thm.} \ref{thm:nph-edgeless}\\
%$\eta$ & \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & {\bf ?} & & &{\bf ?}\\
%${\sf \#agents} + {\sf bundleSize}$& \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & \cellcolor{olivegreen}~\bf{Thm.}\ref{thm:equiavlence} & & & \cellcolor{olivegreen}~{\bf Thm.}\,\ref{thm:equiavlence} \\
%${\sf \# agents} + {\sf bundleSize}+ \eta$ & \cellcolor{lightred} {\bf Obs.}~\ref{obs:wh-eta} & & \dash & & & \dash \\
% $t$ & \cellcolor{olivegreen}~{\bf Thm.}\,\ref{thm:fpt-t} &  & \dash & & & \dash \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Summary of our results of \cffa, where the conflict graph belong to the family $\Co{G}$. \Cy{Lavender}  cell represents polynomial time complexity; {\color{olivegreen} Green} cell and {\color{lightred} Pink} cell denote that the 
%problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively; white cells with {\bf ?} mark denote that the complexity is open; and {\color{yellow} Yellow} cell denote that the respective parameters are not interesting as the problem is either \fpt w.r.t. smaller parameter or for more general graph class.}
%\definecolor{darkyw}{rgb}{0.8,0.6,0}
\begin{figure*}[t!]
%\begin{subfigure}{6cm}
\centering\includegraphics[width=12.4cm,height=2.7cm]{table_fig}
\caption{Summary of our results of \cffa, where the conflict graph belongs to the family $\Co{G}$. {\bf \Cy{Lavender}}  cell represents polynomial time complexity; {\color{olivegreen} {\bf Green}} cell and {\color{lightred} {\bf Pink}} cell denote that the 
problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively; white cells with {\bf ?} mark denotes that the complexity is open; and the {\color{yellow} {\bf Yellow}} cell denotes that the respective parameters are not interesting as the problem is either \fpt w.r.t. smaller parameter or for a more general graph class.}
\label{tab:results}
\end{figure*}%


%\begin{table*}[htp]
%\begin{center}
%\begin{tabular}{|c|c|b |c|c|}
%\hline
%Parameters & Arbitrary & Complete & Cluster & G is {\sf fpt} wrt k \\
%\hline
%\#agents & \cross \cite{deuermeyer1982scheduling} & & \cross {\bf Obs.}~\ref{obs:cluster-2agent}& \cross \cite{deuermeyer1982scheduling}\\
%\#items & \tick~ {\bf Thm.}\,\ref{thm:fpt-with-items} & & \dash & \dash \\
%bundle size & \cross~{\bf Thm.}\,\ref{thm:nph-edgeless} & & \cross~ {\bf Th.}\,\ref{thm:hardnessForcluster} & \cross \\
%$\eta$ & \cross {\bf Obs.}~\ref{obs:wh-eta} & & ? & ?\\
%$\text{\# agents} + \text{bundlesize}$& \cross & & \tick~\bf{Thm.}\ref{thm:equiavlence} & \tick~{\bf Thm.}\,\ref{thm:equiavlence} \\
%$\text{\# agents} + \text{bundlesize} + \eta$ & \cross & & \dash & \dash \\
%distance from $K_{n}$ & \tick~{\bf Thm.}\,\ref{thm:fpt-t} & \dash & \dash & \dash \\
%\hline
%\end{tabular}
%\end{center}
%\caption{\Cy{Light Cyan} represents polynomial time complexity; \tick\ and \cross\ mean the 
%problem is \fpt and \w-hard w.r.t. the parameter in col 1, respectively.}
%
%\label{default}
%\end{table*}%


==> computational_complexity.tex <==
% !TEX root = main.tex

Since the problem coincides with the {\sc Weighted Independent Set} problem (given a vertex weighted graph $G$, the goal is to find an independent set of maximum weight) for $1$ agent~\cite{DBLP:conf/iwoca/ChiarelliKMPPS20}, clearly, it is \nph for all the graph classes for which {\sc Weighted Independent Set} is \nph. 
In this section, we discuss the intractability of the problem for special classes of graph when {\sc  Weighted Independent Set} can be solved in polynomial. %classical complexity of the problem for some special classes of conflict-graphs. 
In particular, we show that the problem is \nph even when the conflict-graph is edgeless and size of every bundle is at most $3$. Clearly, the {\sf NP}-hardness of \cffa for edgeless graphs follows from~\cite{woeginger1997polynomial}. We further show that the problem is \nph for the cluster graph (disjoint union of cliques) with only $3$ cliques. %We further show that the problem is polynomial time solvable for the complete graphs.
%\subsection{Conflict graph is edgeless}\label{sec:nph}
%\input{np-hardness}

%\subsection{Polynomial Time Algorithm}
%\input{clique}

==> intro.tex <==
%!TEX root = main.tex


%\section{Introduction}
%\defproblem{\cffafull (\cffa)}{A set of agents \Co{A}, a set of items \Co{I}, profit function $p_a\colon \I \rightarrow \mathbb{N}$, for each agent $a\in \A$, an integer $\eta$, and a conflict-graph \Co{H}.}{Does there exist an injective function  $\phi \colon \Co{A}  \rightarrow 2^{\Co{I}}$ such that  for every $a\in \Co{A}$, $\phi(a)$ is an independent set in \Co{H}, $\sum_{i\in \phi(a)}p_a(i) \geq \eta$, and $\phi(a)\cap \phi(a') = \emptyset$ for all $\{a,a'\} \subseteq \A$?}
%
%$\Co{A}=\{a_1,\ldots,a_n\}$. 
%We call $\phi$ as an allocation function. For every agent $a\in A$, $\phi(a)$ is the bundle assigned to the agent $a$. The problem is \nph even when $|\Co{A}|=2$ and  \Co{H} is a bipartite graph. 
%\il{Trial~ \cite{election-control}  }
Allocating resources to agents, also called the resource allocation problem, is a universal problem. Indeed, be it government allocating resources to its citizens, or 
school/college administration allocating lecture rooms to classes, or doing time management in daily life is all about matching resources to agents. Thus, unsurprisingly, the problem and its variants have been extensively studied in economics, (computational) social choice theory, game theory, and algorithms and complexity~\cite{woeginger1997polynomial,hummel2022fair,li2021fair,deuermeyer1982scheduling,cheng2022restricted,bezakova2005allocating,kurokawa2018fair,DBLP:conf/atal/EbadianP022,DBLP:conf/atal/BarmanV21,ahmadian2021four,DBLP:conf/iwoca/ChiarelliKMPPS20,DBLP:journals/sigecom/Suksompong21}. There is so much literature on the problem that it is practically impossible to faithfully survey all of them here. % be aware of all of them and to be able to survey them. 

In this paper, we consider a scenario of resource allocation problem, that occurs very naturally in practice.  That is, {\em two resources may not be allocated simultaneously to an agent.}  To further illustrate our point we give couple of examples. 
Consider the classical {\sc Job Scheduling} problem on several non-identical machines (we use the term machines  for workers as well).  Since the machines are non-identical, we can imagine that every machine has different capability to do a job. Suppose every job has a start time and a finish time. Further, a machine can only do one job at a time. So, we can only assign those jobs to a machine whose time intervals do not intersect. The overlap between the time intervals can be modelled as a resource graph as follows: for every job we have a vertex, and if the time interval of two jobs, say $j,j'$, overlaps then we have an edge between the vertices corresponding to jobs $j,j'$. Now, the question is to allocate jobs to machines satisfying some  criteria such that the set of jobs assigned to a machine forms an independent set (i.e., there is no edge between any pair of jobs) in the resource graph. Another scenario is that maybe some resources are incompatible to each other so that they cannot be assigned together. For example, allocation of employees to several projects. For a project, it would be nice to have a team of employees who can collaborate with each other efficiently. In short, our examples show that  there could be interactions and dependencies between the resources, which needs to taken care of. This model has been studied in the literature with some ``fairness" criterion~\cite{hummel2022fair,chiarelli2022fair,li2021fair}

Results on the computational aspect of resource allocation, which also incorporate  interactions and dependencies between the resources, are few and far between. To make our discussion concrete,  we first define the computational problem that abstracts our discussion. 
%

%
\defprob{\cffafull (\cffa)}{A set of agents \Co{A}, a set of items \Co{I}, utility function $\util_a\colon \I \rightarrow \mathbb{N}$, for each agent $a\in \A$, an integer $\eta$, and a graph \Co{H} with vertex set \Co{I}.}{Does there exist an injective function  $\phi \colon \Co{A}  \rightarrow 2^{\Co{I}}$ such that  for every $a\in \Co{A}$, $\phi(a)$ is an independent set in \Co{H}, $\sum_{i\in \phi(a)}\util_a(i) \geq \eta$, and $\phi(a)\cap \phi(a') = \emptyset$ for all $\{a,a'\} \subseteq \A$?}
%
For each $a\in \Co{A}$, we call $\phi(a)$  a {\em bundle} assigned to the agent $a$. We call graph \Co{H}  a {\em conflict graph}.
%
In the literature, \cffa is called conflict free ``maximin fair'' allocation because we are trying to maximize the minimum utility (satisfaction) of agents. Deurmeyer et al.~\cite{deuermeyer1982scheduling} studied \cffa with a different name and showed that the problem is \npc even for $2$ agents and even when \Co{H}  is edgeless (that is, no conflict). Since the problem statement has a conflict graph and we need the subsets of allocated resources to be an independent set in \Co{H}, naturally, the classical {\sc Maximum Weight Independent Set (MWIS)}  problem comes into play. 
In this problem given a graph $G$, a weight function $w: V(G)\rightarrow \mathbb{N}$, and an integer $\eta$, the objective is to test whether there exists an independent set $S$ such that $w(S)=\sum_{v\in S} w(v) \geq \eta$. Let $\mathcal G$ be a family of graphs.
Chiarelli et al.~\cite{DBLP:conf/iwoca/ChiarelliKMPPS20} showed that  if {\sc MWIS} is \npc on $\mathcal G$, then \cffa is \npc, when \Co{H} belongs to the graph class  $\mathcal G$, even when there is one agent.  Consequently, researchers have focused on graph classes on which {\sc MWIS} is polynomial-time solvable.  However, \cffa remains \npc even for bipartite graphs and their {\em line graphs}. Some polynomial time algorithms  for special instances of the problem and polynomial time approximation algorithms are known  for the problem~\cite{deuermeyer1982scheduling,hummel2022fair}. %\todo[inline]{elaborate related work. what are the polytime approximation algorithms or specific tractable cases that are known?}





\subsection{Our Results and Methods} 
We study the problem in the realm of parameterized complexity. 
%\cffa problem is naturally governed by several parameters such as the number of agents (${\sf \#agents}$), the number of items (${\sf \#items}$), the maximum size of a bundle (${\sf bundleSize}$) in the solution, and the utility of any agent $\eta$.  This makes it  a natural candidate for a study from the viewpoint of parameterized complexity. 
The goal of parameterized complexity is to find ways of solving \nph problems more efficiently than brute force: we aim to
restrict the combinatorial explosion to a parameter that is hopefully
much smaller than the input size. Formally, a {\em parameterization}
of a problem is assigning an integer $k$  to each input instance and we
say that a parameterized problem is {\em fixed-parameter tractable
  }(\fpt)  if there is an algorithm that solves the problem in time
$f(k)\cdot |I|^{\Oh(1)}$, where $|I|$ is the size of the input and $f$ is an
arbitrary computable function depending on the parameter $k$
only. Moreover, we will refer to such an algorithm as an \fpt algorithm. For a detailed introduction to the subject, we refer to the textbooks~\cite{ParamAlgorithms15b,fg,downey}.  
%\todo[inline]{The relevance of the parameters that are investigated for CF-FA should be discussed. In what applications do we expect these parameters to be small?}
%In this paper we study \cffa 

\cffa problem is naturally governed by several parameters such as the number of agents (${\sf \#agents}$), the number of items (${\sf \#items}$), the maximum size of a bundle (${\sf bundleSize}$) in the solution, and the utility of any agent $\eta$.  This makes it  a natural candidate for a study from the viewpoint of parameterized complexity. 

\Ma{The parameters under study can indeed be small in real-life scenario. In the example of a job scheduling problem, lecture hall allocation, usually the number of jobs or lecture halls is small, i.e., the number of agents is likely to be small. In the example of school/college admission, the number of school seats is likely to be much smaller than the total number of students. Here, the students are the agents who have preferences over the colleges. The bundle size is also expected to be small in many scenarios due to the scarcity of resources and in the example of the job scheduling problem, due to the limited capacity of the machines, the size of the assigned bundle is kept reasonably small. 
%
The parameters studied in this paper are also natural input/output parameters to study in the paradigm of parameterized complexity. If not very small, we can definitely expect these parameters to be fairly small as compared to the input size. }


%In this paper, 
We study \cffa with two  different sets of parameters\Ma{: input/output parameters, graph structure parameters}.
\subsubsection{Input/Output Parameters}
 The first set of parameters consists of 
$n={\sf \#agents}$, $m={\sf \#items}$, $s={\sf bundleSize}$, and  $\eta$.
With this set of parameters, we obtain the following set of results. 

We first note that due to the known result that \cffa is \npc even for one agent, we cannot even hope for an $(n+m)^{f(n)}$ time algorithm for any function $f$, unless {\sf P=NP}. Thus, no hope of an \fpt algorithm with respect to $n$. Next, we show that \cffa admits an algorithm  with a running time $2^{m}(n+m)^{\Oh(1)}$. One can design an $3^{m}(n+m)^{\Oh(1)}$ time algorithm via a simple dynamic programming, but to design an $2^{m}(n+m)^{\Oh(1)}$ time algorithm we need to use subset convolution-based methods (see~\cite{fomin2013exact} for more details on the topic). This algorithm implies that the problem is \fpt parameterized by $m$ and thus the problem is \fpt with respect to any parameter that depends on $m$ ({\bf \Cref{sec:fpt-input}}).
%
%
%\begin{enumerate}[leftmargin=*]
%\setlength{\itemsep}{-2pt}
%%\item We first study computational complexity of 
%\item The known {\sf NP}-completeness result that \cffa is \npc even for one agent, implies that we cannot even hope for an $(n+m)^{f(n)}$ time algorithm for any function $f$, unless {\sf P=NP}.  
%\item We show that \cffa admits an algorithm  with a running time $2^{m}(n+m)^{\Oh(1)}$. One can design an $3^{m}(n+m)^{\Oh(1)}$ time algorithm via a simple dynamic programming, but to design an $2^{m}(n+m)^{\Oh(1)}$ time algorithm we need to use subset convolution-based methods (see~\cite{fomin2013exact} for more details on the topic). This algorithm implies that the problem is \fpt parameterized by $m$ and thus the problem is \fpt with respect to any parameter that depends on $m$.  ({\bf \Cref{sec:fpt-input}})
%
%\item 
Next, we show that  \cffa is \npc when \Co{H} is edgeless and $\mathsf{bundlesize}$ is three. This implies that we cannot even hope for $(n+m)^{g(\mathsf{bundlesize})}$ time algorithm for any function $g$, unless {\sf P=NP}.  This motivates us to look for the parameter $n+{\sf bundleSize}$ ({\bf \Cref{sec:agents+bundlesize}}). 

\Ma{Before dwelling to other parameters,  we first discuss the  results} given in {\bf \Cref{sec:agents+bundlesize}}. 
%\end{enumerate}
%
%\todo[inline]{Should we move discussion to the section itself?}
In general, hoping that \cffa is \fpt parameterized by $n+{\sf bundleSize}$  is not fruitful, as the problem generalizes the {\sc MWIS} problem. %\Ma{Thus, we consider the special graph classes.}  
In order to incorporate  ${\sf bundleSize}$ as a parameter, we first define the following decision version of \cffa. 
\defprob{\dcffafull \\(\dcffa)}{A set of agents \Co{A}, a set of items \Co{I}, utility function $\util_a\colon \I \rightarrow \mathbb{N}$, for each agent $a\in \A$, integers $s,\eta$, and a graph \Co{H} with vertex set \Co{I}.}{Does there exist an injective function  $\phi \colon \Co{A}  \rightarrow 2^{\Co{I}}$ such that  for every agent $a\in \Co{A}$, bundle $\phi(a)$ is an independent set in \Co{H}, $|\phi(a)|\leq s$, $\sum_{x\in \phi(a)}\util_a(i) \geq \eta$, and $\phi(a)\cap \phi(a') = \emptyset$ for all $\{a,a'\} \subseteq \A$?}


Observe that the ${\sf bundleSize}$ is upper bounded by ${\sf \#items} =m$. Hence, we can run an algorithm for \dcffa, with an increasing value of $s$, from $1$ to $m$, and obtain a parameterized algorithm for \cffa with respect to $n+{\sf bundleSize}$.  
Hence, we can focus on designing an \fpt algorithm for \dcffa.  

If we take a closer look at the hardness proof of \cffa from \mwis, we immediately realize that the hardness of \dcffa comes from the following problem. %, which is of independent interest. 

\defparprob{\mwisfull \\ (\mwis) }{A  graph $G$, positive integers $k$ and $\rho$, a weight function $w: V(G) \rightarrow \mathbb{N}$.}{$k$}{Does there exist an independent set $S$ of size at most $k$ such that 
$w(S)\geq \rho$? That is, $w(S)=\sum_{v\in S}w(v)\geq \rho$.}

%\defparprob{\mwisfull (\mwis) }{A  graph $G$, positive integers $k$ and $\rho$, a weight function $w: V(G) \rightarrow \mathbb{N}$.}{$k$}{Either returns that there is no independent set $S$ of size at most $k$ such that 
%$w(S)\geq \rho$; or returns an independent set $S$  (of any size) such that 
%$w(S)\geq \rho$? Here, $w(S)=\sum_{v\in S}w(v)\geq \rho$.} 
%Does there exist an independent set $S$ of size at most $k$ such that 
%$w(S)\geq \rho$? That is, $w(S)=\sum_{v\in S}w(v)\geq \rho$.}

%\todo[inline]{at most $k$ in the definition.}
A unit weight version of \mwis with $\rho=k$ is a prototype hard problem, known as {\sc Independent Set}, in the field of parameterized complexity,  which in search of \fpt algorithms has been extensively studied on families of graphs that satisfy some structural properties.
Let $\mathcal G$ be a family of {\em hereditary} graphs. That is, if $G\in {\mathcal G} $, then all induced subgraphs of $G$ belong to $\mathcal G$. In other words, $\mathcal G$ is closed under taking induced subgraphs. There are several hereditary graph classes, such that \mwis, when restricted to graphs from these families becomes \fpt. Let $\mathcal G$ be a hereditary family, then \mwisg denotes the restriction of \mwis, where the input graph $G\in \mathcal G$.  Thus a natural question is what happens when in \dcffa, we restrict conflict graphs to a ``tractable hereditary family -- $\mathcal G$'', that is,  \mwisg is \fpt. 
Given a hereditary family $\mathcal G$, we define 
\cffag as follows.  The problem \cffag is similar to \dcffa, except that the conflict graph $\mathcal H$ on the item set $\mathcal I$ belongs to the family $\mathcal G$. %That is, conflict graphs are restricted to belong to $\mathcal G$. 
We wish to point out here that the tractability of \mwisg does not immediately imply tractability of \cffag. Indeed, even if \mwisg is \fpt when parameterized by $k$, we cannot hope for an $(n+m)^{f(n)}$ time algorithm for \dcffa for any function $f$, unless {\sf P=NP}, as the {\sf NP}-hardness of {\sc Independent Set} imply the {\sf NP}-hardness of \cffa even for one agent. Due to \Cref{thm:hardnessForcluster} (explained later), we can also not hope for $s^{f(s)}$ time algorithm for \dcffa for any function $f$, unless {\sf P=NP}, even if  \mwisg is \fpt when parameterized by $k$. So, we study the complexity of the problem with the  combined parameter $n+s$. We show the following result which ties the complexity of \cffag and \mwisg, when parameterized by $n+s$ and $k$, respectively. 


\begin{theorem}
\label{thm:equiavlence}
Let $\mathcal G$  be a hereditary family of graphs. Then, \cffag is \fpt parameterized by $n+s$ if and only if  \mwisg is \fpt parameterized by $k$. 
\end{theorem}

Theorem~\ref{thm:equiavlence} implies that \cffag is \fpt when $ \mathcal G$ are interval graphs, chordal graphs, perfect graphs, planar graphs, bipartite graphs, graphs of bounded degeneracy, to name a few. 
%
%\todo[inline]{Write what all important classes are covered by this. E.g., interval graphs which has application in scheduling problems.}

%\smallskip

\noindent 
{\bf Overview of Theorem~\ref{thm:equiavlence}.} This is one of the main  algorithmic results of this article. The result is obtained by combining the classical color coding technique of Alon-Yuster-Zwick~\cite{alon1995color},  applied on the set of items, together with a dynamic programming algorithm to find a ``colorful solution''. In the dynamic programming phase of the algorithm, we  invoke an \fpt algorithm for \mwisg with respect to $k$.
%
%\todo[inline]{change the following paragraph based on new result. Directly discuss that idea.}

Since there are no known classes of graphs for which \mwisg is \fpt parameterized by $k$, we first identify some such classes. We define an {\em independence friendly class} as follows. Let $f  \colon \mathbb{N} \to \mathbb{N}$ be a monotonically increasing function, that is, invertible. A  
graph class $\mathcal G$ is called {\em $f$-independence friendly class ($f$-ifc)} if $\mathcal G$ is hereditary and for every 
$G\in \mathcal G$ of size $n$ has an independent set of size  $f(n)$. Observe that the families of bipartite graphs, planar graphs, graphs of bounded degeneracy, graphs excluding some fixed clique as an induced subgraphs are $f$-independence friendly classes with appropriate function $f$. For example, for bipartite graphs $f(n)=\nicefrac{n}{2}$ and for $d$-degenerate graphs $f(n)=\nicefrac{n}{(d+1)}$. For  graphs excluding some fixed clique as an induced subgraph, we can obtain the desired $f$ by looking at Ramsey numbers. It is the minimum number of vertices, $n = R(r, s)$, such that all undirected simple graphs of order $n$, contain a clique of size $r$, or an independent set of size $s$. It is known to be upper bounded by $R(r, s) \leq \binom{r + s - 2}{r - 1}$~\cite{jukna2011extremal}. 
%
%We first design an algorithm for the classes of graphs that excluded a fixed graph $H$ as an induced subgraph (call these graphs \emph{$H$-free}). 
%The crucial fact that we use here is that these classes of graphs  contain an independent set whose size ``depends on the size of the input graph'' and it can also be computed in polynomial time. For example, every $n$-vertex planar graph (excludes $K_5$ and $K_{3,3}$) has an independent set of size at least $\nicefrac{n}{4}$ (as a consequence of $4$-Color Theorem).  We first identify the set of vertices, $X$, in the given graph $G$ whose weight is at least $\nicefrac{\rho}{k}$. Note that any independent set of size at most $k$ in the subgraph of $G$ induced on $X$ is the solution. If there is no such independent set, then using the above property on the size of independent set, we know that $|X|$ is bounded by $f(k)$. Furthermore, we know that at least one of the vertex from $X$ is in our solution. So, we can guess the vertex of $X$ in our solution, delete this vertex from the graph,  reduce $k$ by $1$, and iterate. The algorithm stops after $k$ iterations. Thus, we obtain the following result.
We prove the following result for \mwisg when $\Co{G}$ is $f$-ifc. 
\begin{theorem}\label{lem:mwis-degenerate}
Let $\mathcal G$ be $f$-independence friendly class. Then, there exists an algorithm for \mwisg running in time $\Oh((f^{-1}(k))^k\cdot (n+m)^{\Oh(1)})$. %Here $\alpha$ depends on $H$.
%There exists an algorithm that finds an independent set of size at most $k$ with maximum weight in a given $d$-degenerate vertex weighted graph $G$ in 
%running in $\Oh(\binom{k(d+1)}{k}\cdot 2^{{o}(k\cdot(d+1))}\cdot (|V(G)|+|E(G)|) \log |V(G)|)$ time. 
% where $n,m$ denote the number of vertices and edges, respectively, in $G$. 
\end{theorem}
%
We also give a polynomial-time algorithm for \mwisg when $\Co{G}$ is a cluster graph. 


%\todo[inline]{Remove from here}
%There are several families of sparse graphs, such as planar graphs, graphs of bounded genus, graphs of bounded degree, $d$-degenerate graphs, and graphs excluding a fixed biclique as an induced subgraph,  for which {\sc Independent Set}  is \nph, but the problem is known to be \fpt with respect to $k$. These are \fpt because sparse graph classes contain an independent set whose size ``depends on the size of the input graph''. Thus, for these classes of graphs the problem trivially becomes \fpt. For example, every $n$-vertex planar graph has an independent set of size at least $n/4$ (as a consequence of the $4$-Color Theorem). Thus, if $k\leq n/4$, then the problem is polynomial time solvable, else $n\leq 4k$ and  any brute force algorithm is an \fpt algorithm. However, such algorithms do not immediately work for \mwisg, as any independent set of size at most $n/4$ does not satisfy the weight constraint, that we need in order to apply Theorem~\ref{thm:equiavlence}. 
%
%We also give an \fpt algorithm for \mwisg when $\mathcal G$ is a family of $d$-degenerate graphs. 
%%
%For a non-negative integer $d$, a graph $G$ is called a $d$-degenerate graph if every subgraph $G'$ of $G$ has a vertex of degree at most $d$. Every $d$-degenerate graph has a $d$-degeneracy sequence (a $d$-degeneracy sequence of a graph is an ordering of vertices $\sigma$ such that every vertex has at most $d$ neighbors after it in $\sigma$). It is well known that planar graphs, graphs of bounded genus, graphs excluding some fixed graph $H$ as a minor (or topological minor), graphs of bounded expansion, and graphs of bounded degree, are $d$-degenerate graphs, where $d$ depends on the family only. It is known that an $n$-vertex $d$-degenerate graph has an independent set of size $n/(d+1)$, and thus the unweighted version of \mwisg is \fpt, while this does not say anything about \mwisg.  We obtain the following result using the tool of {\em $k$-independence covering family} designed in~\cite{lokshtanov2020covering}. 
%
%\begin{proposition}%\label{lem:mwis-degenerate}
%Let $\mathcal G$ be the family of $d$-degenerate graphs. There exists an algorithm for \mwisg
%%There exists an algorithm that finds an independent set of size at most $k$ with maximum weight in a given $d$-degenerate vertex weighted graph $G$ in 
%running in $\Oh(\binom{k(d+1)}{k}\cdot 2^{{o}(k\cdot(d+1))}\cdot (|V(G)|+|E(G)|) \log |V(G)|)$ time. 
%% where $n,m$ denote the number of vertices and edges, respectively, in $G$. 
%\end{proposition} %\todo{write it as proposition?}


%\todo[inline]{Remove till here!}

Finally, we show that \dcffa  is  \wone with respect to $n+s+\eta$. We reduce it from the {\sc Independent Set} problem.  Given an instance $(G,k)$ of  the {\sc Independent Set}, we can construct an instance of \cffa with only one agent, items as $V(G)$, unit utility function, $\Co{H}=G$, and $s=\eta=k$. Since {\sc Independent Set} is \wone~\cite{downey1995fixed},  we get the following. 

\begin{obs}\label{obs:wh-eta}
\dcffa is \wone with respect to $n+s+\eta$. 
\end{obs}

\subsubsection{Graph Structure Parameters}
Our next set of results is motivated by the following result proved in {\bf \Cref{sec:distance-param}}.
\begin{theorem}($\clubsuit$\footnote{Missing details for results marked with $\clubsuit$ are in supplementary.})\label{thm:poly-clique}
There exists an algorithm that solves \cffa in the polynomial time when the conflict graph is a complete graph.
\end{theorem}
%There is a polynomial time algorithm for \cffa when $\Co{H}$ is a clique.  
This result leads to the following natural question: 

\begin{tcolorbox}[boxsep=5pt,left=5pt,top=5pt,colback=green!5!white,colframe=gray!75!black]
Does \cffa admit a polynomial time  algorithm when $\Co{H}$ is a disjoint union of cliques? 
\end{tcolorbox}

We answer this question negatively by proving the following result, which is due to reduction from \NumMatch. 

\begin{theorem}($\clubsuit$)
\label{thm:hardnessForcluster}
\cffa is \npc when \Co{H} is a cluster graph containing $3$ cliques.
\end{theorem}

Since, an edgeless graph is also a cluster graph, due to \cite{deuermeyer1982scheduling}, we have the following. 
\begin{obs}\label{obs:cluster-2agent}
\cffa is \npc even for $2$ agents when \Co{H} is a cluster graph.
\end{obs}
Next, we design a polynomial time algorithm when a cluster graph contains $2$ cliques and the utility functions are \emph{uniform}, i.e., utility functions are the same for all the agents. In particular, we prove the following result.

%\todo[inline]{The following theorem is new and also needs to be checked.}
\begin{theorem}\label{thm:2cliques}
There exists an algorithm that solves \cffa in polynomial time when \Co{H} is a cluster graph containing $2$ cliques and the utility functions are uniform.
\end{theorem}

In light of Theorem~\ref{thm:poly-clique}, a {\em distance of a graph}  from a complete graph is a natural parameter to study in parameterized complexity.  %This is what we used the term ``distance from tractability''.  
The distance function can be defined in several ways. We define it as follows:  the number of edges, say $t$,  whose addition makes the graph a complete graph.  
We first show a result that gives a {\em subexponential time algorithm}  when the number of agents is constant.
\begin{theorem}\label{thm:fpt-t+n}
There exists an algorithm that solves  \cffa in $\Oh((2t \cdot 2^{2\sqrt{t}}+1)^n(n+m)^{\Oh(1)})$ time, where $t=\binom{n}{2}-|E(\Co{H})|$, the number of edges when added to \Co{H} yields a complete graph.
\end{theorem}
 However, Theorem~\ref{thm:fpt-t+n} is not an \fpt algorithm {\em parameterized by $t$ alone}. To show that the problem is \fpt parameterized by $t$, we obtain the following result. 
\begin{theorem}\label{thm:fpt-t}
There exists an algorithm that solves \cffa in $\Oh((2t)^{t+1}(n+m)^{\Oh(1)})$ time. 
\end{theorem}

Theorem~\ref{thm:fpt-t+n} is obtained by showing that if a graph $G$ can be made into a clique by adding 
at most $t$ edges then the number of independent sets of size at least $2$ is upper bounded by $\Oh(2t \cdot 2^{2\sqrt{t}})$. 

In light of \Cref{thm:poly-clique}, we know that \cffa is polynomial-time solvable when every vertex has degree $n-1$. Next, we show that the problem is also polynomial-time solvable when every vertex has degree $n-2$ and the utility functions are uniform.

\begin{theorem}\label{thm:polytime-n-2}
There exists an algorithm that solves \cffa in polynomial time when every vertex in conflict graph has degree $n-2$ and the utility functions are uniform.
\end{theorem}

Table~\ref{tab:results} summarises all our results. 

\input{table.tex}

%and \ref{thm:fpt-t} are
%\begin{theorem}\label{wh-As}
%\cffa is \wone with respect to $|\Co{A}|+s$, where $\Co{A}$ is the set of agents and $s$ is the maximum size of the bundle assigned to any agent.
%\end{theorem}
%\paragraph{Motivation for Type of Graphs: } Since conflict graph represent conflicts between items, there is no restriction on type of graphs.  It might be anything.  In case of general graphs, the problem is highly intractable. But, in certain situations, we might have specific class of graphs that give us tractability. For example, in case of job scheduling problem, the time-conflict graph is an interval graph. This motivate us to study several special classes of graphs. We are not clear about application of all such graphs, but as mentioned above, it is very well possible that conflict graph has some structure. We can have multiple resources and one resource might have conflict with all resources of same kind. This gives us motivation to study cluster graph. Since resources are generally are not too many, we assume the bound on the number of cliques in cluster graph.


==> prelim.tex <==
%!TEX root = main.tex
%\section{Preliminaries}

Hi add something here?
